Punny Captions: Witty Wordplay in Image Descriptions

Wit is a form of rich interaction that is often grounded in a specific situation (e.g., a comment in response to an event). In this work, we attempt to build computational models that can produce witty descriptions for a given image. Inspired by a cognitive account of humor appreciation, we employ linguistic wordplay, specifically puns, in image descriptions. We develop two approaches which involve retrieving witty descriptions for a given image from a large corpus of sentences, or generating them via an encoder-decoder neural network architecture. We compare our approach against meaningful baseline approaches via human studies and show substantial improvements. We find that when a human is subject to similar constraints as the model regarding word usage and style, people vote the image descriptions generated by our model to be slightly wittier than human-written witty descriptions. Unsurprisingly, humans are almost always wittier than the model when they are free to choose the vocabulary, style, etc.

==> source/discussion.tex <==
\section{Discussion}
Since wit involves unexpectedness, the objective of describing an image in a witty manner often results in a trade-off between the description being witty and the description being relevant to the image. It may be interesting to study how the perceived wittiness of an image description varies as it includes more creative elements and becomes less relevant to the image. 
Another interesting factor that can influence perceived humor is presentation. For instance, the text in cartoons and memes are funny in their characteristic, informal font but may seem boring in other, more ``serious'' font.

\par 
Producing a description for an image that is perceived as witty is challenging because the description must achieve the fine balance between lending itself to easy resolution by the perceiver while not being impossible or too trivial. There are other challenges, however. For instance, automatic image recognition and captioning models, despite the great strides of advancement in recent times, are still imperfect. In our approach, these are cascading sources of error which could adversely affect the perceived wittiness of an image caption.
\par 

In this work, we only consider the use of \emph{words} that are perfect puns. Future work can extend our approach to explore the use of phrase-based and imperfect puns to create alternate interpretations of a sentence. 

\par 
Our approach has no constraints on the modality of the input stimulus. It can be extended to generate witty responses to input stimuli of different modalities, ranging from abstract (cartoon-like) scenes, to describing a given video in a witty manner or to generate witty response (dialog) to a text input.
